On the convergence of Hamiltonian Monte Carlo

This paper discusses the irreducibility and geometric ergodicity of the Hamiltonian Monte Carlo (HMC) algorithm. We consider cases where the number of steps of the symplectic integrator is either fixed or random. Under mild conditions on the potential $\F$ associated with target distribution $\pi$, we first show that the Markov kernel associated to the HMC algorithm is irreducible and recurrent. Under more stringent conditions, we then establish that the Markov kernel is Harris recurrent. Finally, we provide verifiable conditions on $\F$ under which the HMC sampler is geometrically ergodic.

==> degree.tex <==
\section{Definitions and useful results from degree theory}
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> description.tex <==

%However, it is important to note
%that the invariance of π for this kernel is not a sufficient condition
%for the convergence of algorithm.
% However the invariance of
% $\pi$ for this kernel is not a sufficient condition for its convergence. 
% \alain{put a sentence on the fact that most of HMC versions, the
%   invariance is checked and it is not enough for the convergence of
%   the algorithm} 





%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

